Superconstant Inapproximability of Decision Tree Learning

We consider the task of properly PAC learning decision trees with queries. Recent work of Koch, Strassle, and Tan showed that the strictest version of this task, where the hypothesis tree $T$ is required to be optimally small, is NP-hard. Their work leaves open the question of whether the task remains intractable if $T$ is only required to be close to optimal, say within a factor of 2, rather than exactly optimal. We answer this affirmatively and show that the task indeed remains NP-hard even if $T$ is allowed to be within any constant factor of optimal. More generally, our result allows for a smooth tradeoff between the hardness assumption and the inapproximability factor. As Koch et al.'s techniques do not appear to be amenable to such a strengthening, we first recover their result with a new and simpler proof, which we couple with a new XOR lemma for decision trees. While there is a large body of work on XOR lemmas for decision trees, our setting necessitates parameters that are extremely sharp, and are not known to be attainable by existing XOR lemmas. Our work also carries new implications for the related problem of Decision Tree Minimization.

==> IsEdge.tex <==
\section{Constant-error hardness for ${\IsEdge}$}

\begin{theorem}
    Let $T$ be a decision tree for $\IsEdge$ satisfying $\error_{\mathcal{D}}(T,\IsEdge)\le \alpha$ where $\mathcal{D}$ is the canonical hard distribution, then
    $$
    |T|\ge k+(1-2\alpha)m.
    $$
\end{theorem}

\begin{lemma}[Sensitivity of $\IsEdge$]\lnote{Is this a consequence of monotonicity (if so state that), and do we also need this for all subfunctions?}
    For all $x\in \IsEdge^{-1}(1)$, $|\Sens(\IsEdge,x)|=\Cert(\IsEdge,x)$.
\end{lemma}

\begin{proof}
    Let $x\in  \IsEdge^{-1}(1)$ be the indicator for an edge $e=\{u,v\}$. Let $D\sse \zo^n$ denote the set of edge indicators and vertex indicators. Then both $x^{\oplus v},x^{\oplus u}\in D$ are $0$-inputs and all other sensitive neighbors are not in $D$. Therefore, $2=|\Sens(\IsEdge,x)|$. Also, $\{u,v\}$ is a certificate for $x$ so $2=\Cert(\IsEdge,x)$.
\end{proof}


\begin{proposition}
    For all $f:D\to\zo$ with $D\sse\zo^n$, $x\in D$, and restrictions $\pi$ consistent with $x$,
    $$
    |\Sens(f_{\pi},x)|\ge |\Sens(f,x)|-|\pi|.
    $$
\end{proposition}


\section{Constant-error hardness for $\ell\text{-}\IsEdge$}

\begin{theorem}[Hardness for computing $\ell\text{-}\IsEdge$]
    Let $T$ be a decision tree for $\ell\text{-}\IsEdge$ satisfying $\error_{\mathcal{D}}(T,\ell\text{-}\IsEdge)\le \alpha$ where $\mathcal{D}$ is the canonical hard distribution, then
    $$
    |T|\ge (\ell+1)\cdot (k+(1-2\alpha)m).\lnote{Does this mean that we can get any constant error arbitrarily close to $\frac12$? Can we get $\frac12 - o(1)$?}
    $$
\end{theorem}
\calnote{This theorem recovers the constant-error hardness in KST 2023. Note our hard distribution is slightly different (though the support is the same). This version of the theorem and its proof are also simpler than that of KST 2023.}



\section{Constant-error hardness for $\ell\text{-}\IsEdge^{\oplus r}$}

\begin{theorem}[Hardness for computing $\ell\text{-}\IsEdge^{\oplus r}$]
% \label{thm:ellisedge-lb}
    Let $T$ be a decision tree for $\ell\text{-}\IsEdge_G^{\oplus r}$ with $r\ge 2$ which satisfies $\error_{\mathcal{D}}(T,\ell\text{-}\IsEdge^{\oplus r})\le \alpha$ for the canonical hard distribution $\mathcal{D}$, then
    $$
    |T|\ge \big[(\ell+1)(k+m)\big]^r-2\alpha \big[2m(\ell+1)\big]^r
    $$
    where $k$ is the minimum vertex cover size of $G$ and $m$ is the number of edges in $G$.
\end{theorem}


\begin{proof}
    Let $T$ be a decision tree for $\ell\text{-}\IsEdge^{\oplus r}$. Consider $x=(x^{(1)},\ldots,x^{(r)})$ satisfying $\ell\text{-}\IsEdge^{\oplus r}(x^{(i)})=1$. That is each $x^{(i)}$ is the indicator for an edge. The sensitivity of each $x^{(i)}$ is $2(\ell+1)$: $|\Sens(\ell\text{-}\IsEdge, x^{(i)})|=2(\ell+1)$. For any restriction $\pi$, we have $|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|\le |\Sens(\ell\text{-}\IsEdge,x^{(i)})|=2(\ell+1)$ which implies for all $A\sse [r]$:
    \begin{equation}
    \label{eq:prod}
    \prod_{i\in \overline{A}}|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|\ge (2(\ell+1))^{-|{A}|}\prod_{i\in [r]}|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|.
    \end{equation}
    Therefore, we can use \Cref{lem:canonical-xor-error} where $\pi$ is the path followed by $x$ to write
    \begin{align*}
        \Prx_{\by\sim \mu(x)}[\ell\text{-}\IsEdge^{\oplus r}(\by)&\neq T(\by)]\\
        &\ge 2^{-r}\sum_{\substack{A\sse [r]\\\mathrm{Par}(|A|)\neq T(x)}} \prod_{i\in \overline{A}}\frac{|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|}{|\Sens(\ell\text{-}\IsEdge,x^{(i)})|}\tag{\Cref{lem:canonical-xor-error}}\\
        &=2^{-r}\sum_{\substack{A\sse [r]\\\mathrm{Par}(|A|)\neq T(x)}}(2(\ell+1))^{-|\overline{A}|}\prod_{i\in \overline{A}}\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})\tag{$|\Sens(\ell\text{-}\IsEdge,x^{(i)})|=2(\ell+1)$}\\
        &\ge 2^{-r}\sum_{\substack{A\sse [r]\\\mathrm{Par}(|A|)\neq T(x)}} (2(\ell+1))^{-r}\prod_{i\in [r]}|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|\tag{\Cref{eq:prod}}\\
        &=(2(\ell+1))^{-r}\prod_{i\in [r]}|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|\sum_{\substack{A\sse [r]\\\mathrm{Par}(|A|)\neq T(x)}}2^{-r}\\
        &= \frac{1}{2}\cdot(2(\ell+1))^{-r}\prod_{i\in [r]}|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|.\tag{$2^r/2$ many $A\sse[r]$ s.t. $\mathrm{Par}(|A|)\neq T(x)$}
    \end{align*}
\lnote{Re $2^r/2$: doesn't this depend on whether $r$ is even or odd?}    Using this lower bound on the probability $\Prx_{\by\sim \mu(x)}[\ell\text{-}\IsEdge^{\oplus r}(\by)\neq T(\by)]$, we lower bound the total error as:
    \begin{align*}
        \alpha&\ge \Prx_{\bx\sim \mathcal{D}}[\ell\text{-}\IsEdge^{\oplus r}(\bx)\neq T(\bx)]\\
        &= \sum_{x\in \allones(D)}\frac{1}{m^r}\cdot \Prx_{\by\sim \mu(x)}[\ell\text{-}\IsEdge^{\oplus r}(\by)\neq T(\by)]\\
        &\ge \frac{1}{2}\cdot\left(2m(\ell+1)\right)^{-r}\sum_{x\in \allones(D)}\prod_{i\in [r]}|\Sens(\ell\text{-}\IsEdge_{\pi(x)},x^{(i)})|
    \end{align*}
    where $D=\supp(\mathcal{D})$. This in particular implies that
    \begin{equation}
        \label{eq:2alpha}
        2\alpha (2m(\ell+1))^r \ge \sum_{x\in \allones(D)}\prod_{i=1}^r|\Sens(\ell\text{-}\IsEdge_{\pi(x)},x^{(i)})|.
    \end{equation}
    Using the fact that $\Cert(\ell\text{-}\IsEdge,x)=\Sens(\ell\text{-}\IsEdge,x)$ when $x$ is an edge indicator, we have
    \begin{align*}
        \left[(\ell+1)(k+m)\right]^r&\le \dtsize(\ell\text{-}\IsEdge^{\oplus r})\\
        &\le|T|+ \sum_{x\in \allones(D)}\prod_{i=1}^r\Cert(\ell\text{-}\IsEdge_{\pi(x)},x^{(i)})\tag{\Cref{cor:patchup-xor}}\\
        &=|T|+ \sum_{x\in \allones(D)}\prod_{i=1}^r|\Sens(\ell\text{-}\IsEdge_{\pi(x)},x^{(i)})|\tag{$\Sens=\Cert$}\\
        &\le |T|+2\alpha (2m(\ell+1))^r\tag{\Cref{eq:2alpha}}
    \end{align*}
    which implies the desired bound on $T$.
\end{proof}

\violet{
\begin{proof}[Simplified proof]
    We lower bound the total error as:
    \begin{align*}
        \alpha&\ge \Prx_{\bx\sim \mathcal{D}}[\ell\text{-}\IsEdge^{\oplus r}(\bx)\neq T(\bx)]\\
        &= \sum_{x\in \allones(D)}\frac{1}{m^r}\cdot \Prx_{\by\sim \mu(x)}[\ell\text{-}\IsEdge^{\oplus r}(\by)\neq T(\by)]\\
        &\ge \sum_{x\in \allones(D)}\frac{1}{m^r}\cdot \frac{1}{2}\cdot \prod_{i\in [r]}\frac{|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|}{|\Sens(\ell\text{-}\IsEdge,x^{(i)})|} \tag{\Cref{cor:contribution-to-error}}\\
        &=\frac{1}{2}(2m(\ell+1))^{-r}\sum_{x\in \allones(D)}\prod_{i\in [r]}|\Sens(\ell\text{-}\IsEdge_\pi,x^{(i)})|\tag{$|\Sens(\ell\text{-}\IsEdge,x)|=2(\ell+1)$ for all $x\in \ell\text{-}\IsEdge^{-1}(1)$}
    \end{align*}
    where $D=\supp(\mathcal{D})$. This in particular implies that
    \begin{equation}
        \label{eq:2alpha}
        2\alpha (2m(\ell+1))^r \ge \sum_{x\in \allones(D)}\prod_{i=1}^r|\Sens(\ell\text{-}\IsEdge_{\pi(x)},x^{(i)})|.
    \end{equation}
    Using the fact that $\Cert(\ell\text{-}\IsEdge_\pi,x)=\Sens(\ell\text{-}\IsEdge_\pi,x)$ when $x$ is an edge indicator and $\pi$ is a restriction, we have
    \begin{align*}
        \left[(\ell+1)(k+m)\right]^r&\le \dtsize(\ell\text{-}\IsEdge^{\oplus r})\\
        &\le|T|+ \sum_{x\in \allones(D)}\prod_{i=1}^r\Cert(\ell\text{-}\IsEdge_{\pi(x)},x^{(i)})\tag{\Cref{cor:patchup-xor}}\\
        &=|T|+ \sum_{x\in \allones(D)}\prod_{i=1}^r|\Sens(\ell\text{-}\IsEdge_{\pi(x)},x^{(i)})|\tag{$\Sens=\Cert$}\\
        &\le |T|+2\alpha (2m(\ell+1))^r\tag{\Cref{eq:2alpha}}
    \end{align*}
    which implies the desired bound on $T$.
\end{proof}
}

\section{Proofs of \Cref{thm:constant-error-hardness} and \Cref{thm:size-error-tradeoff}}
\calnote{This section still needs to be written.}

We can rewrite the bound in \Cref{thm:ellisedge-lb} as follows\calnote{TODO: add justification for the bound below. We may need to assume that $\alpha$ is small.}
\begin{align*}
    |T|&\ge \big[(\ell+1)(k+m)\big]^r-2\alpha \big[2m(\ell+1)\big]^r\\
    &= \big[(\ell+1)(k+m)\big]^r-\big[(2\alpha)^{1/r}\cdot 2m(\ell+1)\big]^r\\
    &\ge \bigg[(\ell+1)(k+m) - (2\alpha)^{1/r}\cdot 2m(\ell+1)\bigg]^r\\
    &=\bigg[(\ell+1)(k+(1-2\cdot(2\alpha)^{1/r})m)\bigg]^r.
\end{align*}

The above calculation uses the following proposition.
\begin{proposition}
    For all $a,b,r\in\R$ such that $a\ge b$, we have $a^r-b^r\ge (a-b)^r$.
\end{proposition}


Ultimately, for our reduction from vertex cover, we need a lower bound on $T$ of the form $\bigg[(\ell+1)(k+(1-\delta)m)\bigg]^r$ where $\delta>0$ is a small constant that depends on the degree of $G$. So we will need to choose the error parameter $\alpha=2^{-\Theta(r)}$ small enough so that $2\cdot(2\alpha)^{1/r}=\delta$. 

\section{Tightness of our XOR lemma: a constructive upper bound for computing the XOR of $r$ copies of $\IsEdge$}

\paragraph{High level idea of the construction.}{
 The idea is to fully compute $\IsEdge$ on each input block until $\tau$ edge inputs have been seen for some threshold $\tau\in [r]$. That is, the decision tree is ``Shaltiel-like'' in the sense that if the input is ``easy'' (meaning it doesn't have too many edges in it) then the decision tree fully computes the parity and otherwise if it discovers that the input is hard, it gives up.
}

\begin{theorem}[Tightness of XOR lemma]
\label{thm:tight}
    Let $G$ be a graph with $m$ edges and let $k$ denote the minimum vertex cover size of $G$ and suppose that $m\ge (1+\delta)k$ for some constant $\delta>0$. Then, for every $r\in \N$, is an $\alpha>0$ such that the following holds. There is a decision tree $T$ satisfying $\Prx_{\bx\sim\mathcal{D}}[T(\bx)\neq \IsEdge^{\oplus r}(\bx)]\le \alpha$ and whose size is
    $$
    |T|\le \bigg[k+(1-\Theta(2^r\alpha))m\bigg]^r.
    $$
\end{theorem}

\paragraph{Some remarks on \Cref{thm:tight}.}{
Checking whether an edge is present in an input block requires $k$ queries. So roughly speaking, the savings obtained by the cutoff strategy is proportional to $m$, the number of queries it takes to actually identify the edge. To ensure that the savings of this is large enough, we need $m$ to be slightly bigger than $k$ by a constant factor. This assumption can be made without loss of generality, as it is possible to show that it is NP-hard to approximate vertex cover to within a constant factor on constant-degree graphs satisfying $m\ge 2k$.

There is some slack in this tightness result due to the constant in front of the $2^r\alpha$ term. Nonetheless, the example shows that the exponential dependence on $r$ in the lower bound is necessary.
}

\paragraph{Main lemmas.}
Let $T^\star$ with cutoff parameter $\tau$ be the following decision tree for $\IsEdge^{\oplus r}$. For $i=1,\ldots, r$, start by computing $\IsEdge(x^{(i)})$ using $k+m$ queries. If $\IsEdge(x^{(i)})=1$, i.e. $x^{(i)}$ is an edge input, and there have been a total of $\tau$ or more edge inputs in previous blocks, then halt and output $1$. Otherwise, continue. 

\begin{lemma}[Size of $T^\star$]
    For all $\tau\in [r]$, we have
    $$
    |T^\star|\le \sum_{i=0}^{\tau}\binom{r}{i}k^{r-i}m^i.
    $$
\end{lemma}


\begin{lemma}[Error of $T^\star$]
    The error of $T^\star$ in computing $\IsEdge^{\oplus r}$ is bounded by
    $$
    \error_{\mathcal{D}}(T^\star,\IsEdge^{\oplus r})\le \Prx_{x\sim\mathcal{D}}[\#\text{ edge inputs in }x\text{ is more than }\tau].
    $$
\end{lemma}

\newpage 


==> body-of-paper-arxiv.tex <==
\section{Patching up a decision tree: Proof of \Cref{lem:patchup-intro}}
% We refer the reader to \Cref{sec:prelims} for an overview of the notation and terminology we use throughout the paper. 
We start with the following claim about building a decision tree from scratch using certificates. 

% See \Cref{subsec:zero-error-patch-up} for the proof.

\begin{claim}[Building a decision tree out of certificates]
\label{claim:zero-error-patch-up}
    Let $f:D\to\zo$ be a function with $D\sse \zo^n$, then
    $$
    \dtsize(f)\le 1+\sum_{x\in f^{-1}(1)}\Cert(f,x).
    $$
\end{claim}

\begin{proof}
    Let $T$ be the decision tree built iteratively by the following procedure. In the first iteration, pick an arbitrary $x\in f^{-1}(1)$ and fully query the indices in $\Cert(f,x)$. Let $T_i$ be the tree formed after the $i$th iteration. Then $T_{i+1}$ is formed by choosing $x\in f^{-1}(1)$ which has not been picked in a previous iteration. Then, at the leaf reached by $x$ in $T_i$, fully query the indices in $\Cert(f,x)$ (ignoring those indices which have already been queried along the path followed by $x$ in $T_i$). Repeating this for $|f^{-1}(1)|$ steps, yields a decision tree with at most $\sum_{x\in f^{-1}(1)}\Cert(f,x)$ \textit{internal nodes}. Therefore, the number of leaves is at most $1+\sum_{x\in f^{-1}(1)}\Cert(f,x)$. 
        
        It remains to show that this tree exactly computes $f$. Specifically, we'll argue that $f_\pi$ is the constant function for every path $\pi$ in the decision tree. If not, then there is an $x\in f^{-1}(1)$ so that $x$ follows the path $\pi$ and $f_\pi$ is nonconstant. But this is a contradiction since $\pi$ consists of a certificate of $x$ by construction.
\end{proof}

The next lemma shows that we can patch up a decision tree by querying certificates. This recovers \Cref{lem:patchup-intro} in the setting where $D=\zo^n$.

\begin{lemma}[Patch-up with respect to $1$-inputs]
\label[lemma]{lem:patch-up-dt}
    Let $f:D\to\zo$ be a function with $D\sse \zo^n$ and let $T$ be a decision tree, then
    $$
    \dtsize(f)\le |T|+\sum_{x\in f^{-1}(1)}\Cert(f_{\pi(x)},x)
    $$
\end{lemma}

\begin{proof}
    Let $\Pi$ denote the set of paths in $T$. Then,
    \begin{align*}
        \dtsize(f)&\le \sum_{\pi\in\Pi}\dtsize(f_\pi)\\
        &\le \sum_{\pi\in\Pi}\left(1+\sum_{x\in f_\pi^{-1}(1)}\Cert(f_\pi,x)\right)\tag{\Cref{claim:zero-error-patch-up}}\\
        &= |T|+\sum_{\pi\in\Pi}\sum_{x\in f_\pi^{-1}(1)}\Cert(f_\pi,x)\tag{$|\Pi|=|T|$}\\
        &=|T|+\sum_{x\in f^{-1}(1)}\Cert(f_{\pi(x)},x).
    \end{align*}
    The last equality follows from the fact that the set of paths $\pi\in \Pi$ partition $f^{-1}(1)$.
\end{proof}

% ----------------------------------------HARD DISTRIBUTION LEMMA----------------------------

\section{Hard distribution lemma: Proof of \Cref{lem:hard-distribution-intro}}

\Cref{lem:hard-distribution-intro} is proved for the \textit{canonical hard distribution} for a partial function $f:D\to\zo$. 

\begin{definition}[Canonical hard distribution]
\label[definition]{def:canonical-hard-distribution}
    For a function $f:D\to\zo$ with $D\sse \zo^n$, the canonical hard distribution, $\mathcal{D}_f$, is defined via the following experiment
    \begin{itemize}
        \item sample $\bx\sim f^{-1}(1)$ u.a.r.
        \item with probability $1/2$, return $\by\sim\Sens(f,\bx)$ u.a.r.
        \item with probability $1/2$, return $\bx$.
    \end{itemize}
\end{definition} 
When $f$ is clear from context, we simply write $\mathcal{D}$.
We use the canonical hard distribution to prove the following result which recovers \Cref{lem:hard-distribution-intro} in the setting where $D=\zo^n$. 

% See \Cref{sec:hard-dist-lemma} for the proof.

\begin{lemma}[Hard distribution lemma]
\label[lemma]{lem:hard-distribution-lemma}
    Let $f:D\to\zo$ be a nonconstant function for $D\sse \zo^n$. Then for all $C\sse f^{-1}(1)$, there exists a distribution $\mathcal{D}$ over $C$ and and all of its sensitive neighbors such that for any decision tree $T$, we have
    $$
    \mathrm{error}_{\mathcal{D}}(T,f)\ge \frac{1}{2|C|\Sens(f)}\sum_{x\in C}|\Sens(f_{\pi(x)},x)|.
    $$
\end{lemma}

First we prove a claim which counts the error under $\mathcal{D}$ conditioned on the $1$-input obtained in the first sampling step. 
\begin{claim}[Error with respect to the canonical hard distribution conditioned on a $1$-input]
\label[claim]{lem:error-conditioned-on-one}
    Let $T$ be a decision tree, $f:D\to\zo$ be a function, and let $\mathcal{D}$ be the canonical hard distribution. For all $x\in f^{-1}(1)$, 
    $$
    \Prx_{\bz\sim\mathcal{D}_f}[T(\bz)\neq f(\bz)\mid \text{ first sampling }x\text{ from }f^{-1}(1)]\ge \frac{1}{2}\cdot\frac{|\Sens(f_{\pi(x)},x)|}{\max\{1,|\Sens(f,x)|\}}.
    $$
\end{claim}

\begin{proof}
    If $|\Sens(f,x)|=0$ then $|\Sens(f_{\pi(x)},x)|=0$. And if the RHS is $0$ then the bound is vacuously true. Assume that $\Sens(f_{\pi(x)},x)\neq \varnothing$. Both $x$ and all $y\in \Sens(f_{\pi(x)},x)$ follow the same path in $T$ and have the same leaf label. Since $f(x)=1$ and $f(y)=0$, we can write
    \begin{align*}
        \Prx_{\bz\sim\mathcal{D}_f}\big[T(\bz)\neq f(\bz)\mid \textnormal{first sampling }x&\textnormal{ from }f^{-1}(1)\big]\\
        \ge \min\bigg\{&\Prx_{\bz\sim\mathcal{D}_f}\big[\bz=x\mid \textnormal{first sampling }x\textnormal{ from }f^{-1}(1)\big],\\
        &\Prx_{\bz\sim\mathcal{D}_f}\big[\bz\in\Sens(f_{\pi(x)},x)\mid \textnormal{first sampling }x\textnormal{ from }f^{-1}(1)\big]\bigg\}\\
        =\min\bigg\{&\frac{1}{2},\frac{1}{2}\cdot \frac{|\Sens(f_{\pi(x)},x)|}{|\Sens(f,x)|}\bigg\}\ge \frac{1}{2}\cdot\frac{|\Sens(f_{\pi(x)},x)|}{|\Sens(f,x)|}
        % \ge\min\bigg\{&1-p,\frac{p}{\Sens(f)}\bigg\}\tag{$|\Sens(f_{\pi(x)},x)|\ge 1$ and $|\Sens(f,x)|\le \Sens(f)$}
    \end{align*}
    where the inequality follows from the fact that the probability of an error is lower bounded by the probability that $\bz=x$ when the label for the path in $T$ is $0$ and is lower bounded by the probability that $\bz\in\Sens(f_{\pi(x)},x)$ when the label for the path is $1$. Note that if $\Sens(f_{\pi(x)},x)\neq \varnothing$ then necessarily $|\Sens(f,x)|\ge 1$ and $\max\{1,|\Sens(f,x)|\}=|\Sens(f,x)|$. Therefore, the proof is complete.
\end{proof}


\begin{proof}[Proof of \Cref{lem:hard-distribution-lemma}]
    We prove the statement for $C=f^{-1}(1)$. If $C\neq f^{-1}(1)$, we can consider the function $f:C\cup C'\to \zo$ where $C'$ denotes the set of sensitive neighbors of strings in $C$, and the same proof holds. Let $\mathcal{D}$ denote the distribution from \Cref{def:canonical-hard-distribution} and notice that the support of this distribution is $C$ and all of its sensitive neighbors. We have
    \begin{align*}
        \mathrm{error}_{\mathcal{D}}(T,f)&=\Prx_{\bz\sim\mathcal{D}}[T(\bz)\neq f(\bz)]\\
        &=\sum_{x\in C}\frac{1}{|C|}\cdot \Prx_{\bz\sim\mathcal{D}}[T(\bz)\neq f(\bz)\mid \text{ first sampling }x\text{ from }f^{-1}(1)]\\
        &\ge \frac{1}{2|C|}\sum_{x\in C}\frac{|\Sens(f_{\pi(x)},x)|}{\max\{1,|\Sens(f,x)|\}}\tag{\Cref{lem:error-conditioned-on-one}}\\
        &\ge \frac{1}{2|C|\cdot\Sens(f)}\sum_{x\in C}|\Sens(f_{\pi(x)},x)|\tag{$\max\{1,|\Sens(f,x)|\}\le \Sens(f)$ for all $x$}
    \end{align*}
    where the last step uses the fact that $\Sens(f)\ge 1$ since $f$ is nonconstant. In particular, we have that $\max\{1,|\Sens(f,x)|\}\le \Sens(f)$ for all $x$.
\end{proof}



% ----------------------------------------ISEDGE AND HARDNESS OF LEARNING----------------------------

\section{Hardness of learning via $\ell$-$\IsEdge$}

We are interested in the following learning task.

\begin{tcolorbox}[colback = white,arc=1mm, boxrule=0.25mm]
\vspace{3pt} 
{\sc DT-Learn$(s,s',\eps)$:}  Given queries to an unknown function $f : \zo^n \to \zo$, random samples from a distribution $\mathcal{D}$ over $\zo^n$, parameters $s,s'\in \N$ and $\eps \in (0,1)$, and the promise that $f$ is a size-$s$ decision tree, construct a size-$s'$ decision tree $T$ that is $\eps$-close to $f$ under $\mathcal{D}$.
\vspace{3pt}
\end{tcolorbox}
\medskip

The main theorem of this section is the following reduction from approximating {\sc Vertex Cover} to {\sc DT-Learn}. This theorem recovers, via a simpler proof, the main reduction in \cite{KST23}, while also achieving a better dependence on the {\sc Vertex Cover} approximation factor. Later, we build on this reduction to prove our main result \Cref{thm:main}.

\begin{theorem}[Reduction from {\sc Vertex Cover} to {\sc DT-Learn}]
\label{thm:KST}
    If there is a time-$t(n,1/\eps)$ algorithm solving {\sc DT-Learn}$(s,(1+\delta)s,\eps)$ over $n$-variable functions for any $\eps>0$, $s=O(n)$, and $\delta>0$, then {\sc Vertex Cover} can be $(1+\delta')$-approximated on degree-$d$, $n$-vertex graphs in randomized time $O(n^2\cdot t(n^2,1/\eps))$ for any $\delta' > (\delta+4\eps)d+\delta$. 
\end{theorem}

At a high level, \Cref{thm:KST} works by taking a graph $G$, and defining an ``amplified'' version of the edge indicator function for $G$ (recall \Cref{def: isedge}). This function is called $\ell$-$\IsEdge$ and is formally defined as follows (see also \cite{KST23}).


\begin{definition}[The $\ell$-amplified {$\IsEdge$} function]\label[definition]{def:ell-isedge} Let $G = (V,E)$ be an $n$-vertex graph and $\ell \in \N$. The {\sl $\ell$-amplified edge indicator function of $G$} is the function 
\[ \ell\text{-}\mathrm{\IsEdge}_G : \zo^n \times (\zo^n)^\ell \to \zo\] 
 defined as follows: $\ell\text{-}\mathrm{\IsEdge}_G(v^{(0)},v^{(1)},\ldots,v^{(\ell)}) = 1$ if and only if 
\begin{enumerate} 
\item $\mathrm{\IsEdge}_G(v^{(0)}) = 1$ (i.e.~$v^{(0)} = \Ind[e]$ for some $e\in E$), and
\item $v_{i}^{(1)} = \cdots = v_i^{(\ell)} = 1$ for all $i\in [n]$ such that $v_i^{(0)} = 1$. 
\end{enumerate} 
We write $\ell\text{-}\Ind[e] \in (\zo^n)^{\ell+1}$ for the \textit{generalized edge indicator} $(\Ind[e],\ldots,\Ind[e])$. Note that $\ell\text{-}\mathrm{\IsEdge}(\ell\text{-}\Ind[e]) = 1$.
\end{definition}



\subsection{Decision tree size upper bound for $\ell\text{-}\mathrm{\IsEdge}_G$: First part of \Cref{claim:slight-inapprox} }

The upper bound in \Cref{claim:slight-inapprox} follows from \cite[Theorem 2]{KST23}: 

\begin{theorem}[Upper bound on decision tree size of $\ell$-$\IsEdge$ {\cite[Theorem 2]{KST23}}]
\label{thm:ell-isedge-ub}
    Let $G$ be an $n$-vertex, $m$-edge graph with a vertex cover of size $k$. Then, there is a decision tree $T$ computing $\ell\text{-}\IsEdge_G:\zo^{n\ell+n}\to\zo$ whose size satisfies
    $$
    |T|\le (\ell+1)(k+m)+mn
    $$
    and $T$ can be computed in polynomial-time given $G$ and a size-$k$ vertex cover of $G$.
\end{theorem}
The last part of \Cref{thm:ell-isedge-ub}, the constructivity of $T$, is implicit in the proof of \cite[Theorem 2]{KST23}, but is made explicit in their paper when proving Lemma 5.2 (see Section 5.3 of \cite{KST23}).

\subsection{Decision tree size lower bound for $\ell\text{-}\mathrm{\IsEdge}_G$: Second part of \Cref{claim:slight-inapprox} }

The lower bound in \Cref{claim:slight-inapprox} is proved with respect to the canonical hard distribution for $\ell\text{-}\mathrm{\IsEdge}_G$:
\begin{definition}[Canonical hard distribution for $\ell\text{-}\IsEdge$]
    For a graph $G$, we write $\ell\text{-}\mathcal{D}_G$ to denote the canonical hard distribution of $\ell\text{-}\IsEdge$ and $\ell\text{-}{D}_G=\supp(\ell\text{-}\mathcal{D}_G)$ to denote the support of the canonical hard distribution. As per \Cref{def:canonical-hard-distribution}, this distribution is defined via the experiment
    \begin{itemize}
        \item sample $\ell\text{-}\ind[e]$ u.a.r.~among all generalized edge indicators;
        \item with probability $1/2$, return $\by$ sampled u.a.r.~from the set of sensitive neighbors:\\ $\Sens(\ell\text{-}\IsEdge,\ell\text{-}\ind[e])$ $=\{\ell\text{-}\ind[e]^{\oplus i}\mid i\text{ is a }1\text{-coordinate of }\ell\text{-}\ind[e]\}$; and
        \item with probability $1/2$, return $\ell\text{-}\ind[e]$.
    \end{itemize}
\end{definition}

\begin{lemma}[Decision tree size lower bound for computing $\ell\text{-}\IsEdge$]
\label[lemma]{lem:ell-isedge-lb}
    Let $T$ be a decision tree for $\ell\text{-}\IsEdge_G$ satisfying $\error_{\ell\text{-}\mathcal{D}_G}(T,\ell\text{-}\IsEdge)\le \eps$, then
    $$
    |T|\ge (\ell+1)\cdot (k'+(1-4\eps)m)
    $$
    where $m$ is the number of edges of $G$ and $k'$ is the vertex cover size of $G$.
\end{lemma}

We obtain \Cref{lem:ell-isedge-lb} using an application of the general size lower bound from \Cref{lem:patch-up-dt,lem:hard-distribution-lemma}. 

% See \Cref{subsec:ell-isedge-lb} for the proof.

First, we give a basic zero-error lower bound on $\ell\text{-}\IsEdge$ and observe some properties about the sensitivity and certificate complexity of $\ell\text{-}\IsEdge$ in \Cref{lem:ell-isedge-lb-zero-error,prop:sens-ell-isedge,prop:sens-equals-cert}, respectively.

\begin{lemma}[Zero-error lower bound for $\ell\text{-}\IsEdge_G$; see {\cite[Claim 6.6]{KST23}}]
\label[lemma]{lem:ell-isedge-lb-zero-error}
    Let $G$ be an $n$-vertex, $m$-edge graph where every vertex cover has size at least $k'$. Then, any decision tree $T$ computing $\ell\text{-}\IsEdge_G:\ell\text{-}{D}_G\to\zo$ over $\ell\text{-}{D}_G$, the support of the canonical hard distribution, must have size
    $$
    |T|\ge (\ell+1)(k'+m).
    $$
\end{lemma}

\begin{proof}
    The same lower bound is proved in Claim 6.6 of \cite{KST23} under a slightly different subset of inputs. Specifically, they prove $\dtsize(\ell\text{-}\IsEdge_G)\ge (\ell+1)(k'+m)$ where $\ell\text{-}\IsEdge_G:D'\to\zo$ for the set $D'=\ell\text{-}{D}_G\cup\{0^{n+\ell n}\}$ which adds the all 0s input. This small difference doesn't change the lower bound since any decision tree $T$ computing $\ell\text{-}\IsEdge_G$ over the set $\ell\text{-}{D}_G$ also computes it over $D'$. Indeed, every $1$-input to $\ell\text{-}\IsEdge_G$ is sensitive on every $1$-coordinate and so if $T$ satisfies $T(x)=\ell\text{-}\IsEdge_G(x)$ for every $x\in \ell\text{-}{D}_G$, then it must query every $1$-coordinate of each $1$-input. Therefore, we can assume without loss of generality that $T(0^{n+\ell n})=0$.
\end{proof}


\begin{proposition}[Sensitivity of $\ell\text{-}\IsEdge_G$]
\label{prop:sens-ell-isedge}
    For a graph $G$, $\ell\ge 1$, and $\ell\text{-}\IsEdge_G:\ell\text{-}{D}_G\to\zo$, we have
    $$
    \Sens(\ell\text{-}\IsEdge_G)=2(\ell+1).
    $$
\end{proposition}

\begin{proof}
    Let $\ell\text{-}\ind[e]$ be an edge indicator for an edge $e\in E$. Let $i\in [n\ell+n]$ denote the index of a $1$-coordinate of $\ell\text{-}\ind[e]$. By definition, there are $2(\ell+1)$ many such $i$ and each $i$ is sensitive: $\ell\text{-}\IsEdge_G(\ell\text{-}\ind[e]^{\oplus i})=0$. Therefore, $|\Sens(\ell\text{-}\IsEdge_G,\ell\text{-}\ind[e])|=2(\ell+1)$. Conversely, for every sensitive neighbor $\ell\text{-}\ind[e]^{\oplus i}$, we have $\Sens(\ell\text{-}\IsEdge_G,\ell\text{-}\ind[e]^{\oplus i})=\{\ell\text{-}\ind[e]\}$ and so $|\Sens(\ell\text{-}\IsEdge_G,\ell\text{-}\ind[e]^{\oplus i})|=1$. Thus the overall sensitivity is $\Sens(\ell\text{-}\IsEdge_G)=2(\ell+1).$
\end{proof}


\begin{proposition}[Sensitivity equals certificate complexity of $1$-inputs]
    \label[proposition]{prop:sens-equals-cert}
    Let $G$ be a graph and $\ell\text{-}\IsEdge:\ell\text{-}{D}_G\to\zo$, the corresponding edge function. For all edge indicators $x=\ell\text{-}\ind[e]$ and for all restrictions $\pi$, we have
    $$
    \Cert(\ell\text{-}\IsEdge_\pi,x)=|\Sens(\ell\text{-}\IsEdge_\pi,x)|.
    $$
\end{proposition}

\begin{proof}
    By definition $|\Sens(\ell\text{-}\IsEdge_\pi,x)|$ is the number of $1$-coordinates in $x$ which are not restricted by $\pi$. The set of $1$-coordinates of $x$ not restricted by $\pi$ forms a certificate of $\ell\text{-}\IsEdge_\pi$ since fixing these coordinates forces $\ell\text{-}\IsEdge$ to be the constant $1$-function. It follows that $\Cert(\ell\text{-}\IsEdge_\pi,x)=|\Sens(\ell\text{-}\IsEdge_\pi,x)|$.
\end{proof}

\begin{proof}[Proof of \Cref{lem:ell-isedge-lb}]
    For a graph consisting of $m$ edges, the number of $1$-inputs to $\ell\text{-}\IsEdge:\ell\text{-}{D}_G\to\zo$ is $m$. Therefore,
    \begin{align*}
        \eps &\ge \frac{1}{2m\cdot\Sens(\ell\text{-}\IsEdge)}\sum_{x\in \ell\text{-}\IsEdge^{-1}(1)}|\Sens(\ell\text{-}\IsEdge_{\pi(x)},x)|\tag{\Cref{lem:hard-distribution-lemma}}\\
        &=\frac{1}{2m\cdot \Sens(\ell\text{-}\IsEdge)}\sum_{x\in \ell\text{-}\IsEdge^{-1}(1)}\Cert(\ell\text{-}\IsEdge_{\pi(x)},x)\tag{\Cref{prop:sens-equals-cert}}\\
        &\ge \frac{1}{2m\cdot \Sens(\ell\text{-}\IsEdge)}\left(\dtsize(\ell\text{-}\IsEdge,\ell\text{-}{D}_G)-|T|\right).\tag{\Cref{lem:patch-up-dt}}
    \end{align*}
    Rearranging the above, we obtain
    \begin{align*}
    |T|&\ge \dtsize(\ell\text{-}\IsEdge,\ell\text{-}{D}_G)-2\eps m\cdot\Sens(\ell\text{-}\IsEdge)\\
    &\ge(\ell+1)(k'+m)-2\eps m\cdot\Sens(\ell\text{-}\IsEdge)\tag{\Cref{lem:ell-isedge-lb-zero-error}}\\
    &=(\ell+1)(k'+m)-4\eps m(\ell+1)\tag{\Cref{prop:sens-ell-isedge}}
    \end{align*}
    which completes the proof.
\end{proof}





\subsection{Putting things together to prove \Cref{thm:KST}}
 
 The following key lemma is used in the analysis of correctness for the reduction in \Cref{thm:KST}. It follows from \Cref{claim:slight-inapprox} and a careful choice of parameters. 
 
 % We defer the proof to \Cref{subsec:technical-kst}.

\begin{lemma}[Main technical lemma]
\label[lemma]{lem:technical-kst}
For all $\delta,\delta',\eps >0$ and $d,k\ge 1$, the following holds. Given a constant degree-$d$ graph $G$ with $m$ edges and parameter $k$, there is a choice of $\ell=\Theta(|G|)$ and a polynomial-time computable quantity $s\in\N$ such that so long as $\delta'>(\delta+4\eps)d+\delta$ and $dk\ge m$ we have:
\begin{itemize}
    \item \textbf{Yes case}: if $G$ has a vertex cover of size at most $k$, then there is a decision tree of size at most $s$ which computes $\ell\text{-}\IsEdge:\zo^{n\ell+n}\to\zo$; and
    \item \textbf{No case}: if every vertex cover of $G$ has size at least $(1+\delta')k$, then $(1+\delta)s<|T|$ for any decision tree $T$ with $\error_{\ell\text{-}\mathcal{D}_G}(T,\ell\text{-}\IsEdge)\le \eps$.
\end{itemize}
\end{lemma}

This lemma is a consequence of the following proposition along with the upper and lower bounds we have obtained for $\ell\text{-}\IsEdge$. The proposition is a calculation involving the parameters that come into play in \Cref{lem:technical-kst}. We state it on its own, since we will reuse the calculation later when proving \Cref{thm:main-general}.

\begin{proposition}
\label[proposition]{prop:inequality}
    For all $\delta,\delta',\alpha>0$ and $\ell,m,n,k,d\ge 1$ satisfying $m\le dk$ and $\delta'>(\delta+\alpha)d+\delta+\frac{(1+\delta)mn}{k(\ell+1)}$, we have
    $$
    (1+\delta)\left[(\ell+1)(k+m)+mn\right]<(\ell+1)\left[(1+\delta')k+(1-\alpha) m\right].
    $$
\end{proposition}

\begin{proof}
    The proof is a calculation. We can write
    \begin{align*}
        (1+\delta')k-(1+\delta)k&=(\delta'-\delta)k\\
        &>\left(\delta+(\delta+\alpha)d+\frac{(1+\delta)mn}{k(\ell+1)}-\delta\right)k\tag{Assumption on $\delta'$}\\
        &=(\delta+\alpha)dk+\frac{(1+\delta)mn}{\ell+1}\\
        &\ge (\delta+\alpha)m+\frac{(1+\delta)mn}{\ell+1}\tag{$m\le dk$}\\
        &=(1+\delta)m-(1-\alpha)m+\frac{(1+\delta)mn}{\ell+1}.
    \end{align*}
    Therefore, rearranging we obtain
    $$
    (1+\delta)\left[(\ell+1)(k+m)+mn\right]<(\ell+1)\left[(1+\delta')k+(1-\alpha) m\right]
    $$
    which completes the proof. 
\end{proof}

\begin{proof}[Proof of \Cref{lem:technical-kst}]
    Given a degree-$d$, $m$-edge, $n$-vertex graph $G$ and parameter $k$, we choose $\ell=\Theta(n)$ so that $\delta'>(\delta+4\eps)d+\delta+\frac{(1+\delta)mn}{k(\ell+1)}$ and set $s=(\ell+1)(k+m)+mn$. Note that such an $\ell$ exists since $k=\Theta(n)$ for constant-degree graphs. We now prove the two points separately.

    \paragraph{Yes case.}{
        In this case, we have by \Cref{thm:ell-isedge-ub} that there is a decision tree $T$ computing $\ell\text{-}\IsEdge:\zo^{n\ell+n}\to\zo$ whose size satisfies
        $$
        |T|\le (\ell+1)(k+m)+mn=s.
        $$
    }
    \paragraph{No case.}{
        Let $T$ be a decision tree satisfying $\error_{\ell\text{-}\mathcal{D}_G}(T,\ell\text{-}\IsEdge)\le \eps$. Then, using our assumptions on the parameters: 
        \begin{align*}
        (1+\delta)s&=(1+\delta)\left[(\ell+1)(k+m)+mn\right]\tag{Definition of $s$}\\
            &<(\ell+1)\left[(1+\delta')k+(1-4\eps) m\right]\tag{\Cref{prop:inequality} with $\alpha=4\eps$}\\
            &\le|T|\tag{\Cref{lem:ell-isedge-lb} with $k'=(1+\delta')k$}.
        \end{align*}
    }
    We've shown the desired bounds in both the Yes and No cases so the proof is complete.
\end{proof}


\Cref{thm:KST} follows in a straightforward way from \Cref{lem:technical-kst}. 

% We defer the proof of it to \Cref{subsec:KST}.

\begin{proof}[Proof of \Cref{thm:KST}]
Let $G$ be a constant degree-$d$, $n$-vertex graph and $k\in \N$, a parameter. Let $\mathcal{A}$ be the algorithm for {\sc DT-Learn} from the theorem statement. We'll use $\mathcal{A}$ to approximate {\sc Vertex Cover} on $G$.

\paragraph{The reduction.}{
First, we check whether $dk\ge m$. If $dk<m$, our algorithm outputs ``No'' as $G$ cannot have a vertex cover of size at most $k$. Otherwise, we proceed under the assumption that $dk\ge m$. Let $s\in \N$ be the quantity from \Cref{lem:technical-kst}. We will run $\mathcal{A}$ over the distribution $\ell\text{-}\mathcal{D}_G$ and on the function $\ell\text{-}\IsEdge_G:\zo^{N}\to\zo$ where $\ell$ is as in \Cref{lem:technical-kst}. Note that $N=n\ell+n=O(n^2)$ and $s=O(n^2)=O(N)$. See \Cref{fig:solving vc with dt learn} for the exact procedure we run. 
}

\begin{figure}[h!]
\begin{tcolorbox}[colback = white,arc=1mm, boxrule=0.25mm]
\vspace{3pt}
$\textsc{Vertex Cover}(k,(1+\delta')\cdot k)$:
\begin{itemize}[leftmargin=20pt,align=left]
\item[\textbf{Given:}] $G$, an $m$-edge degree-$d$ graph over $n$ vertices and $k\in \N$
\item[\textbf{Run:}]\textsc{DT-Learn}$(s,(1+\delta)\cdot s,\eps)$ for $t(N,1/\eps)$ time steps providing the learner with
\begin{itemize}[align=left,labelsep*=0pt]
    \item \textit{queries}: return $\ell\text{-}{\mathrm{\IsEdge}}(v^{(0)},\ldots,v^{(\ell)})$ for a query $(v^{(0)},\ldots,v^{(\ell)})\in\zo^N$; and
    \item \textit{random samples}: return $(\bv^{(0)},\ldots,\bv^{(\ell)})\sim\ell\text{-}\mathcal{D}_G$ for a random sample.
\end{itemize}
\item[$T_{\text{hyp}}\leftarrow$ decision tree output of the learner]
\item[$\eps_{\text{hyp}}\leftarrow \mathrm{error}_{\ell\text{-}\mathcal{D}_G}(T_{\text{hyp}},\ell\text{-}{\mathrm{\IsEdge}})$]
\item[\textbf{Output:}] \textsc{Yes} if and only if $|T_{\text{hyp}}|\le (1+\delta)\cdot s$ and $\eps_{\text{hyp}}\le \eps$
\end{itemize}
\vspace{3pt}
\end{tcolorbox}
\medskip
\caption{Using an algorithm for \textsc{DT-Learn} to solve \textsc{Vertex Cover}.}
\label{fig:solving vc with dt learn}
\end{figure}


\paragraph{Runtime.}{
Any query to $\ell\text{-}{\mathrm{\IsEdge}}$ can be answered in $O(N)$ time. Similarly, a random sample can be obtained in $O(N)$ time. The algorithm uses $O(N\cdot t(N,1/\eps))$ time to run \textsc{DT-Learn}. Finally, computing $\mathrm{error}_{\ell\text{-}\mathcal{D}_G}(T_{\text{hyp}},\ell\text{-}{\mathrm{\IsEdge}})$ takes $O(N^2)$. Since $t(N,1/\eps)\ge N$, the overall runtime is $O(N\cdot t(N,1/\eps))=O(n^2t(n^2,1/\eps))$. 
}


\paragraph{Correctness.}{
Correctness follows from \Cref{lem:technical-kst}. Specifically, in the \textbf{Yes case}, if $G$ has a vertex cover of size at most $k$, then there is a decision tree of size at most $s$ computing $\ell\text{-}{\mathrm{\IsEdge}}$.  Therefore, by the guarantees of {\sc DT-Learn}, we have $|T_{\text{hyp}}|\le (1+\delta)\cdot s$ and $\eps_{\text{hyp}}\le \eps$ and our algorithm correctly outputs ``Yes''.  

In the \textbf{No case}, every vertex cover of $G$ has size at least $(1+\delta')k$. If $\eps_{\text{hyp}}>\eps$ then our algorithm for {\sc Vertex Cover} correctly outputs ``No''. Otherwise, assume that $\eps_{\text{hyp}}\le \eps$. Then, \Cref{lem:technical-kst} ensures that $(1+\delta)s<|T_{\text{hyp}}|$ and so our algorithm correctly outputs ``No'' in this case as well.
}
This completes the proof.
\end{proof}


% ----------------------------------------PATCHUP FOR XOR----------------------------

\section{Patching up a decision tree for $f^{\oplus r}$: Proof of \Cref{lem:patchup-xor-intro}}

The following lemma recovers \Cref{lem:patchup-xor-intro} by setting $D=\zo^n$. 

% See \Cref{sec:patchup-xor} for the proof.

\begin{lemma}[XOR-ed version of patchup lemma, formal statement of \Cref{lem:patchup-xor-intro}]
\label[lemma]{lem:patchup-xor}
    Let $T$ be a decision tree and $f:D\to\zo$ be a nonconstant function for $D\sse \zo^n$, then
    $$
    \dtsize(f^{\oplus r})\le |T|+2^{r}\sum_{\substack{x\in f^{-1}(1)^r \\ f_{\pi(x)}^{\oplus r} \textnormal{ is nonconstant} }}\prod_{i=1}^r\max\{1,\Cert(f_{\pi(x)},x^{(i)})\}.
    $$
\end{lemma}

For the lemma, we require the following generalization of a result from~\cite{Sav02}. Savick\'y proved that for functions $f_1:\zo^n\to\zo$ and $f_2:\zo^n\to\zo$, it holds that $\dtsize(f_1\oplus f_2)\ge \dtsize(f_1)\cdot\dtsize(f_2)$ \cite[Lemma 2.1]{Sav02}. We will use the following analogous statement for partial functions.

\begin{theorem}[Generalization of Savick\'y \citep{Sav02}]
    \label{thm:zero-error-xor}
    Let $f^{(1)},\ldots, f^{(r)}$ be functions, $f^{(i)}:D^{(i)}\to\zo$ with $D^{(i)}\sse\zo^{n^{(i)}}$ for each $i=1,\ldots, r$. Then,
    $$
    \dtsize(f^{(1)}\oplus\cdots\oplus f^{(r)})=\prod_{i=1}^r \dtsize(f^{(i)}).
    $$
\end{theorem}

\input{fig-stacked}

\begin{proof}
    First, the upper bound $\dtsize(f^{(1)}\oplus\cdots\oplus f^{(r)})\le \prod_{i=1}^r \dtsize(f^{(i)})$ follows by considering the decision tree for $f^{(1)}\oplus\cdots\oplus f^{(r)}$ which sequentially computes $f^{(i)}(x)$ for each $i=1,\ldots, r$ using a decision tree of size $\dtsize(f^{(i)})$. See \Cref{fig:stacked} for an illustration of this decision tree.

    The lower bound is by induction on $\sum_{i\in [r]} n^{(i)}$, the total number of input variables. In the base case, $n=0$ and the bound is trivially true: the constant function requires a decision tree of size $1$. For the inductive step, let $T$ be a decision tree for $f^{(1)}\oplus\cdots\oplus f^{(r)}$ of size $\dtsize(f^{(1)}\oplus\cdots\oplus f^{(r)})$, and let $x_{j}$ be the variable queried at the root. Assume without loss of generality that $x_{j}$ belongs to $f^{(1)}$. The subfunctions computed at the left and right branches of the root of $T$ are $f^{(1)}_{x_j\leftarrow 0}\oplus\cdots\oplus f^{(r)}$ and $f^{(1)}_{x_j\leftarrow 1}\oplus\cdots\oplus f^{(r)}$, respectively. Each is a function on $\left(\sum_{i\in [r]} n^{(i)}\right)-1$ many variables and so we can apply the inductive hypothesis. Therefore:
    \begin{align*}
        \dtsize(f^{(1)}\oplus\cdots\oplus f^{(r)})&=|T|\\
        &\ge\dtsize(f^{(1)}_{x_j\leftarrow 0}\oplus\cdots\oplus f^{(r)})+\dtsize(f^{(1)}_{x_j\leftarrow 1}\oplus\cdots\oplus f^{(r)})\tag{Root of $T$ is $x_j^{(1)}$}\\
        &\ge \dtsize(f^{(1)}_{x_j\leftarrow 0})\prod_{i=2}^r \dtsize(f^{(i)})+\dtsize(f^{(1)}_{x_j\leftarrow 1})\prod_{i=2}^r \dtsize(f^{(i)})\tag{Inductive hypothesis}\\
        &=\left(\dtsize(f^{(1)}_{x_j\leftarrow 0})+\dtsize(f^{(1)}_{x_j\leftarrow 1})\right)\prod_{i=2}^r \dtsize(f^{(i)})\\
        &\ge \prod_{i=1}^r \dtsize(f^{(i)})
    \end{align*}
    where the last step follows from the fact that $\dtsize(f^{(1)}_{x_j\leftarrow 0})+\dtsize(f^{(1)}_{x_j\leftarrow 1})\ge \dtsize(f^{(1)})$. Indeed, one can construct a decision tree for $f^{(1)}$ of size $\dtsize(f^{(1)}_{x_j\leftarrow 0})+\dtsize(f^{(1)}_{x_j\leftarrow 1})$ by querying $x_j$ at the root and on the left branch placing a tree for $f^{(1)}_{x_j\leftarrow 0}$ and on the right branch placing a tree for $f^{(1)}_{x_j\leftarrow 1}$.
\end{proof}


\begin{proof}[Proof of \Cref{lem:patchup-xor}]
    Let $\Pi$ denote the set of paths. For each path $\pi\in \Pi$, we write $\pi^{(i)}$ for $i\in [r]$ to denote the part of $\pi$ corresponding to the $i$th block of input variables. This way, the restricted function $f_\pi^{\oplus r}$ corresponds to the function $f_{\pi^{(1)}}\oplus\cdots\oplus f_{\pi^{(r)}}$ Then we have
\begin{align*}
    \dtsize(f_\pi^{\oplus r})&\le \sum_{\pi\in \Pi}\dtsize(f_\pi^{\oplus r})\\
    &= \sum_{\substack{\pi\in\Pi\\ f_\pi^{\oplus r} \text{ is constant}}}\dtsize(f_\pi^{\oplus r})+\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\dtsize(f_\pi^{\oplus r})\\
    &= |T|+\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\dtsize(f_\pi^{\oplus r})\tag{$\dtsize(f_\pi^{\oplus r})=1$ when $f_\pi^{\oplus r}$ is constant}\\
    &= |T|+\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\prod_{i=1}^r\dtsize(f_{\pi^{(i)}})\tag{\Cref{thm:zero-error-xor}}\\
    &\le |T|+\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\prod_{i=1}^r\left(1+\sum_{x: f_{\pi^{(i)}}(x)=1}\Cert(f_{\pi^{(i)}},x)\right)\tag{\Cref{claim:zero-error-patch-up}}
\end{align*}

We use the fact that $1+a\le 2\max\{1,a\}$ for all $a\in\R$ to rewrite the above in a simpler form, while suffering a factor of $2^r$:
\begin{align*}
    |T|+&\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\prod_{i=1}^r\left(1+\sum_{x: f_{\pi^{(i)}}(x)=1}\Cert(f_{\pi^{(i)}},x)\right)\\
    &\le |T|+\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\prod_{i=1}^r\left(2\max\{1,\sum_{x: f_{\pi^{(i)}}(x)=1}\Cert(f_{\pi^{(i)}},x)\}\right)\\
    &\le |T|+2^r\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\prod_{i=1}^r\left(\sum_{x: f_{\pi^{(i)}}(x)=1}\max\{1,\Cert(f_{\pi^{(i)}},x)\}\right)\\
    &= |T|+2^r\sum_{\substack{\pi\in \Pi\\ f_\pi^{\oplus r} \text{ is nonconstant}}}\sum_{x^{(1)}:f_{\pi^{(1)}}(x^{(1)})=1}\cdots\sum_{x^{(r)}:f_{\pi^{(r)}}(x^{(r)})=1}\prod_{i=1}^r\max\{1,\Cert(f_{\pi^{(i)}},x^{(i)})\}\\
    &=|T|+2^r\sum_{\substack{x\in f^{-1}(1)^r \\ f_{\pi(x)}^{\oplus r}\textnormal{ is nonconstant} }}\prod_{i=1}^r\max\{1,\Cert(f_{\pi^{(i)}},x^{(i)})\}
\end{align*}
    where the last equality follows from the fact that $\Pi$ partitions the input space and so for every $x\in f^{-1}(1)^r$ there is exactly one path $\pi\in \Pi$ such that $f_{\pi^{(i)}}(x^{(i)})=1$ for all $i\in [r]$.
\end{proof}

% ----------------------------------------HARD DISTRIBUTION FOR XOR----------------------------
\section{Hard distribution lemma for $f^{\oplus r}$: Proof of \Cref{lem:hard-distribution-xor-intro}}

The following lemma recovers \Cref{lem:hard-distribution-xor-intro} by setting $D=\zo^n$. 

% See \Cref{sec:hard-distribution-xor} for the proof.
\begin{lemma}[Hard distribution lemma for $f^{\oplus r}$]
\label[lemma]{lem:hard-distribution-lemma-xor}
    Let $T$ be a decision tree, $f:D\to\zo$ be a nonconstant function and let $C \sse f^{-1}(1)$. There is a distribution $\mathcal{D}$ over the inputs in $C$ and their sensitive neighbors such that for all $r\ge 1$,
    $$
    \mathrm{error}_{\mathcal{D}^{\otimes r}}(T,f^{\oplus r})\ge \left(\frac{1}{2|C|\Sens(f)}\right)^r\sum_{\substack{x\in C^r\\ \Sens(f_{\pi(x)}^{\oplus r},x)\neq\varnothing}}\prod_{i=1}^r\max\{1,\Sens(f_{\pi(x)}^{(i)},x^{(i)})\}.
    $$
\end{lemma}

First, we prove the following claim.
\begin{claim}[Error of $f^{\oplus r}$ conditioned on an input]
\label[claim]{lem:xor-conditional-error}
    Let $T$ be a decision tree, $r\ge 1$, $f:D\to\zo$ be a nonconstant function, $x\in f^{-1}(1)^r$, $\mathcal{D}$ be the canonical hard distribution, and $\pi$ be the path followed by $x$ in $T$ and assume that $\Sens(f_{\pi(x)}^{\oplus r},x)\neq\varnothing$, then
    $$
    \Prx_{\bz\sim \mathcal{D}^{\otimes r}}[f^{\oplus r}(\bz)\neq T(\bz)\mid \text{ first sampling }x]\ge 2^{-r}\prod_{i=1}^r\frac{\max\{1,|\Sens(f_\pi^{(i)},x^{(i)})|\}}{\max\{1,|\Sens(f^{(i)},x^{(i)})|\}}.
    $$
\end{claim}

\begin{proof}
    Let $y\in \Sens(f_\pi^{\oplus r},x)$ and let $j\in [r]$ be such that $y^{(j)}\in \Sens(f_\pi^{(j)},x^{(j)})$. Since $f^{\oplus r}(y)\neq f^{\oplus r}(x)$, we have
    \begin{align*}
        \Prx_{\bz\sim \mathcal{D}^{\otimes r}}&[f^{\oplus r}(\bz)\neq T(\bz)\mid \text{ first sampling }x]\\
        &\ge \min\big\{ \Prx_{\bz\sim \mathcal{D}^{\otimes r}}[\bz=x\mid \text{ first sampling }x],\\
        &\qquad\Prx_{\bz\sim \mathcal{D}^{\otimes r}}[\bz=(x^{(1)},...,y,...,x^{(r)})\text{ for }y\in\Sens(f_\pi^{(j)},x^{(j)})\mid \text{ first sampling }x] \big\}\tag{Either $x$ or $(x^{(1)},...,y,...,x^{(r)})$ makes an error}\\
        &= \min\left\{2^{-r},2^{-(r-1)}\frac{|\Sens(f_\pi^{(j)},x^{(j)})|}{|\Sens(f^{(j)},x^{(j)})|}\right\}\tag{Definition of $\mathcal{D}^{\otimes r}$}\\
        &\ge 2^{-r}\frac{|\Sens(f_\pi^{(j)},x^{(j)})|}{|\Sens(f^{(j)},x^{(j)})|}\\
        &\ge 2^{-r}\frac{|\Sens(f_\pi^{(j)},x^{(j)})|}{|\Sens(f^{(j)},x^{(j)})|}\cdot\prod_{i\in [r]\setminus\{j\}}\frac{\max\{1,|\Sens(f_\pi^{(i)},x^{(i)})|\}}{\max\{|\Sens(f^{(i)},x^{(i)})|\}}\tag{${\max\{1,|\Sens(f_\pi^{(i)},x^{(i)})|\}}\le \max\{1,|\Sens(f^{(i)},x^{(i)})|\} $ for all $i$}\\
        &=2^{-r}\prod_{i=1}^r\frac{\max\{1,|\Sens(f_\pi^{(i)},x^{(i)})|\}}{\max\{1,|\Sens(f^{(i)},x^{(i)})|\}}\tag{$|\Sens(f_\pi^{(j)},x^{(j)})|\neq 0$ by assumption}.
    \end{align*}
\end{proof}


We can now prove the main result of this section.

\begin{proof}[Proof of \Cref{lem:hard-distribution-lemma-xor}]
    As in the case of \Cref{lem:hard-distribution-lemma}, we assume without loss of generality that $C=f^{-1}(1)$. We lower bound the error as follows 
    \begin{align*}
        \eps&\ge \Prx_{\bz\sim\mathcal{D}^{\otimes r}}[T(\bz)\neq f^{\oplus r}(\bz)]\\
        &=\sum_{\substack{x\in C^r \\ \Sens(f_{\pi(x)}^{\oplus r},x)\neq\varnothing }}\frac{1}{|C|^r}\cdot\Prx_{\bz\sim\mathcal{D}^{\otimes r}}[T(\bz)\neq f^{\oplus r}(\bz)\mid \text{ first sampling }x\text{ from } C^r]\\
        &\ge (2|C|)^{-r}\sum_{\substack{x\in C^r \\ \Sens(f_{\pi(x)}^{\oplus r},x)\neq\varnothing }}\prod_{i=1}^r\frac{\max\{1,|\Sens(f_\pi^{(i)},x^{(i)})|\}}{\max\{1,|\Sens(f^{(i)},x^{(i)})|\}}\tag{\Cref{lem:xor-conditional-error}}\\
        &\ge (2|C|\cdot\Sens(f))^{-r}\sum_{\substack{x\in C^r \\ \Sens(f_{\pi(x)}^{\oplus r},x)\neq\varnothing }}\prod_{i=1}^r\max\{1,|\Sens(f_\pi^{(i)},x^{(i)})|\}\tag{$|\Sens(f^{(i)},x^{(i)})|\le\Sens(f)$}
    \end{align*}
    which completes the proof.
\end{proof}


% ----------------------------------------XOR of ISEDGE AND HARDNESS OF LEARNING------------------------

\section{Hardness of learning via $\ell\text{-}\IsEdge^{\oplus r}$}

The main theorem of this section is the following reduction from approximating {\sc Vertex Cover} to {\sc DT-Learn}. This reduction enables us to prove \Cref{thm:main,thm:main-general}.

\begin{theorem}[Main reduction from vertex cover to {\sc DT-Learn}]
\label{thm:dt-learn-xor}
    For all $r\ge 1$, $\eps<2^{-3r}$, and $A>1$ the following holds. If there is a time $t(s,1/\eps)$ algorithm for solving {\sc DT-Learn}$(s,A\cdot s,\eps)$ on $n$-variable functions with $s=O(n^r)$, then {\sc Vertex Cover} can be $(1+\delta')$-approximated on degree-$d$, $n$-vertex graphs in randomized time $O(rn^2\cdot t(n^{2r},1/\eps))$ for any $\delta'>(A^{1/r}-1+\eps^{1/r}\cdot 8)d+A^{1/r}-1$.
\end{theorem}

The proof largely follows the steps in proving \Cref{thm:KST} where the lower bound is obtained using a combination of \Cref{lem:hard-distribution-lemma-xor,lem:patchup-xor}.

% We defer the proof to \Cref{sec:dt-learn-xor}.

Before proving this theorem, we establish a few properties of $\ell\text{-}\IsEdge^{\oplus r}$ which will be helpful for our analysis.

\begin{theorem}[Decision tree size lower bound for computing $\ell\text{-}\IsEdge^{\oplus r}$]
\label{thm:ellisedge-lb-xor}
Let $T$ be a decision tree for $\ell\text{-}\IsEdge_G^{\oplus r}$ with $\ell, r\ge 1$. Let $k$ be the minimum vertex cover size of $G$ and let $m$ denote the number of edges of $G$. Then, if $\error_{\ell\text{-}\mathcal{D}_G^{\otimes r}}(T,\ell\text{-}\IsEdge^{\oplus r})\le \eps$ for the canonical hard distribution $\ell\text{-}\mathcal{D}_G$, we have
    $$
    |T|\ge \big[(\ell+1)(k+m)\big]^r-\eps \big[8m(\ell+1)\big]^r
    $$
\end{theorem}

\begin{proof}
    Since $\ell\text{-}\IsEdge$ has $m$ many $1$-inputs over the dataset $\ell\text{-}D_G$ and $\Sens(\ell\text{-}\IsEdge)=2(\ell+1)$, we have
    \begin{align*}
        \eps&\ge \left(\frac{1}{4m(\ell+1)}\right)^r\sum_{\substack{x\in \ell\text{-}D_G^r\\ \Sens(\ell\text{-}\IsEdge_{\pi(x)}^{\oplus r},x)\neq\varnothing}}\prod_{i=1}^r\max\{1,\Sens(\ell\text{-}\IsEdge_{\pi(x)}^{(i)},x^{(i)})\}\tag{\Cref{lem:hard-distribution-lemma-xor}}\\
        &=\left(\frac{1}{4m(\ell+1)}\right)^r\sum_{\substack{x\in \ell\text{-}D_G^r\\ \Sens(\ell\text{-}\IsEdge_{\pi(x)}^{\oplus r},x)\neq\varnothing}}\prod_{i=1}^r\max\{1,\Cert(\ell\text{-}\IsEdge_{\pi(x)}^{(i)},x^{(i)})\}\tag{\Cref{prop:sens-equals-cert}}\\
        &\ge \left(\frac{1}{4m(\ell+1)}\right)^r\sum_{\substack{x\in \ell\text{-}D_G^r\\ \ell\text{-}\IsEdge_{\pi(x)}^{\oplus r} \text{ is nonconstant}    }}\prod_{i=1}^r\max\{1,\Cert(\ell\text{-}\IsEdge_{\pi(x)}^{(i)},x^{(i)})\}\\
        &\ge \left(\frac{1}{8m(\ell+1)}\right)^r(\dtsize(\ell\text{-}\IsEdge^{\oplus r})-|T|)\tag{\Cref{lem:patchup-xor}}.
    \end{align*}
    In this derivation, we used the fact that if an input $x\in \ell\text{-}D_G^r$ is such that $\ell\text{-}\IsEdge_{\pi(x)}^{\oplus r}$ is nonconstant, then it must be the case that there is some block $i\in [r]$ where the path $\pi$ does not fully restrict the sensitive coordinates in the edge indicator for block $i$, and therefore it must also be the case that $\Sens(\ell\text{-}\IsEdge_{\pi(x)}^{\oplus r},x)\neq\varnothing$. Now, we can rearrange this lower bound on $\eps$ to obtain:
    \begin{align*}
        |T|&\ge\dtsize(\ell\text{-}\IsEdge^{\oplus r})-\eps \big[8m(\ell+1)\big]^r\\
        &=\dtsize(\ell\text{-}\IsEdge)^r-\eps \big[8m(\ell+1)\big]^r\tag{\Cref{thm:zero-error-xor}}\\
        &\ge \big[(\ell+1)(k+m)\big]^r-\eps \big[8m(\ell+1)\big]^r\tag{\Cref{lem:ell-isedge-lb-zero-error}}
    \end{align*}
    which completes the proof.
\end{proof}

The following proposition allows us to translate the above lower bound into a slightly simpler form.
\begin{proposition}
\label{prop:inequality-for-xor}
    For all $a,b,r>0$ such that $a\ge b$, we have $a^r-b^r\ge (a-b)^r$.
\end{proposition}

\begin{proof}
    Since $a\ge b$, we have
    $$
    1\ge \left(1-\frac{b}{a}\right)^r+\left(\frac{b}{a}\right)^r.
    $$
    Multiplying both sides of the inequality by $a^r$ and rearranging gives the desired bound.
\end{proof}

With \Cref{thm:ellisedge-lb-xor,prop:inequality-for-xor}, we are able to prove the main technical lemma used for our reduction.

\begin{lemma}[Main technical lemma for \Cref{thm:dt-learn-xor}]
\label{lem:technical-xor}
For all $\delta,\delta',\eps >0$ and $d,k,r\ge 1$, the following holds. Given a constant degree-$d$ graph $G$ with $m$ edges, $n$ vertices, and parameter $k$, there is a choice of $\ell=\Theta(n)$ and a polynomial-time computable quantity $s\in\N$ such that so long as $\delta'>(\delta+8\eps^{1/r})d+\delta$, $dk\ge m$, and $\eps<2^{-3r}$ we have:
\begin{itemize}
    \item \textbf{Yes case}: if $G$ has a vertex cover of size at most $k$, then there is a decision tree of size at most $s$ which computes $\ell\text{-}\IsEdge^{\oplus r}:\zo^{r(n\ell+n)}\to\zo$; and
    \item \textbf{No case}: if every vertex cover of $G$ has size at least $(1+\delta')k$, then $(1+\delta)^r s<|T|$ for any decision tree $T$ with $\error_{\ell\text{-}\mathcal{D}_G^{\otimes r}}(T,\ell\text{-}\IsEdge)\le \eps$.
\end{itemize}
\end{lemma}

\begin{proof}
    Given a degree-$d$, $m$-edge, $n$-vertex graph $G$ and parameter $k$, we choose $\ell=\Theta(n)$ so that $\delta'>(\delta+8\eps^{1/r})d+\delta+\frac{(1+\delta)mn}{k(\ell+1)}$ and set $s=\left[(\ell+1)(k+m)+mn\right]^r$. Note that such an $\ell$ exists since $k=\Theta(n)$ for constant-degree graphs. We now prove the two points separately.

    \paragraph{Yes case.}{
        In this case, we have
        \begin{align*}
            \dtsize(\ell\text{-}\IsEdge^{\oplus r})&=\dtsize(\ell\text{-}\IsEdge)^r\tag{\Cref{thm:zero-error-xor}}\\
        &\le \left[(\ell+1)(k+m)+mn\right]^r=s\tag{\Cref{thm:ell-isedge-ub}}.
        \end{align*}
    }
    \paragraph{No case.}{
        In this case, let $T$ be a decision tree with $\error_{\ell\text{-}\mathcal{D}_G^{\otimes r}}(T,\ell\text{-}\IsEdge)\le \eps$. Then we have
        \begin{align*}
            (1+\delta)^r s&=\bigg[(1+\delta)[(\ell+1)(k+m)+mn]\bigg]^r\\
            &<\left[(\ell+1)(1+\delta')k+(\ell+1)(1-8\eps^{1/r}) m\right]^r\tag{\Cref{prop:inequality} with $\alpha=8\eps^{1/r}$}\\
            &\le \big[(\ell+1)(k+m)\big]^r-\eps \big[8m(\ell+1)\big]^r\tag{\Cref{prop:inequality-for-xor}}\\
            &\le |T|\tag{\Cref{thm:ellisedge-lb-xor}}.
        \end{align*}
    }
    We've shown the desired bounds in both the Yes and No cases so the proof is complete.
\end{proof}


\begin{proof}[Proof of \Cref{thm:dt-learn-xor}]
Let $\mathcal{A}$ be the algorithm for {\sc DT-Learn} from the theorem statement. Given an $n$-vertex, $m$-edge graph $G$ of constant degree $d$, we'll use $\mathcal{A}$ to approximate {\sc Vertex Cover} on $G$.

\paragraph{The reduction.}{
    First, we check whether $dk\ge m$. If $dk<m$, our algorithm outputs ``No'' as $G$ cannot have a vertex cover of size at most $k$ (see \Cref{fact:constant degree graphs have large vc size}). Otherwise, we proceed under the assumption that $dk\ge m$. Let $s\in \N$ be the quantity from \Cref{lem:technical-xor}. We run $\mathcal{A}$ over the distribution $\ell\text{-}\mathcal{D}_G^{\otimes r}$ and on the function $\ell\text{-}\IsEdge^{\oplus r}:\zo^N\to\zo$ where $\ell$ is as in \Cref{lem:technical-xor}. Note that $N=r\cdot(n\ell+n)=O(rn^2)$ and $s=O(n^{2r})$. See \Cref{fig:solving vc with dt learn xor} for the exact procedure we run.
        % Given an $n$-vertex, $m$-edge graph $G$ of constant degree $d$, and a parameter $k$, we construct the following instance of {\sc DT-Learn}. Fix $\ell=\Theta(n)$ as in \Cref{lem:technical-xor}. Consider the function $\ell\text{-}\IsEdge^{\oplus r}_{G}:\zo^{rN}\to\zo$ where $N=n+\ell n$. Let $\mathcal{D}$ be the canonical hard distribution for $\ell\text{-}\IsEdge_G$. We run the algorithm for {\sc DT-Learn} on $\ell\text{-}\IsEdge^{\oplus r}_{G}$ over the distribution $\mathcal{D}^{\otimes r}$ with $s=\left[(\ell+1)(k+m)+mn\right]^r\le O(N^r)$ for $t(s)\le t(N^r)$ time steps with error parameter $\eps$ from the theorem statement. Let $T$ denote the decision tree output by the learner. Our algorithm for vertex cover outputs ``Yes'' if and only if $|T|\le A\cdot\left[(\ell+1)(k+m)+mn\right]^r$ and the error of $T$ with $\ell\text{-}\IsEdge^{\oplus r}_{G}$ over $\mathcal{D}^{\otimes r}$ is less than $\eps$. 
}

\begin{figure}[!ht]
\begin{tcolorbox}[colback = white,arc=1mm, boxrule=0.25mm]
\vspace{3pt}
$\textsc{Vertex Cover}(k,(1+\delta')\cdot k)$:
\begin{itemize}[leftmargin=20pt,align=left]
\item[\textbf{Given:}] $G$, an $m$-edge degree-$d$ graph over $n$ vertices and $k\in \N$
\item[\textbf{Run:}]\textsc{DT-Learn}$(s,A\cdot s,\eps)$ for $t(s,1/\eps)$ time steps providing the learner with
\begin{itemize}[align=left,labelsep*=0pt]
    \item \textit{queries}: return $\ell\text{-}{\mathrm{\IsEdge}}^{\oplus r}(x)$ for a query $x\in\zo^N$; and
    \item \textit{random samples}: return $\bx\sim\ell\text{-}\mathcal{D}_G^{\otimes r}$ for a random sample.
\end{itemize}
\item[$T_{\text{hyp}}\leftarrow$ decision tree output of the learner]
\item[$\eps_{\text{hyp}}\leftarrow \mathrm{error}_{\ell\text{-}\mathcal{D}_G^{\otimes r}}(T_{\text{hyp}},\ell\text{-}{\mathrm{\IsEdge}}^{\oplus r})$]
\item[\textbf{Output:}] \textsc{Yes} if and only if $|T_{\text{hyp}}|\le A\cdot s$ and $\eps_{\text{hyp}}\le \eps$
\end{itemize}
\vspace{3pt}
\end{tcolorbox}
\medskip
\caption{Using an algorithm for \textsc{DT-Learn} on $\ell\text{-}{\mathrm{\IsEdge}}^{\oplus r}$ to solve \textsc{Vertex Cover}.}
\label{fig:solving vc with dt learn xor}
\end{figure}

    \paragraph{Runtime.}{Any query to $\ell\text{-}\IsEdge^{\oplus r}_{G}$ can be answered in $O(N)$ time. Similarly, a random sample can be obtained in $O(N)$ time. The algorithm requires time $O(N\cdot t(N^r,1/\eps))$ to run the learner and then $O(N^2)$ time to compute $\dist_{\mathcal{D}^{\otimes r}}(T,\ell\text{-}\IsEdge^{\oplus r}_{G})$. This implies an overall runtime of $O(N\cdot t(N^r,1/\eps))=O(rn^2\cdot t(n^{2r},1/\eps))$.}

    \paragraph{Correctness.}{
        If we let $\delta\coloneqq A^{1/r}-1$, then the assumption of the theorem statement is that $\delta'>(\delta+8\eps^{1/r})d+\delta$. Therefore, we are able to apply \Cref{lem:technical-xor} from which we deduce correctness.
        
        In the \textbf{Yes case}, if $G$ has a vertex cover of size at most $k$, then there is a decision tree of size at most $s$ computing $\ell\text{-}\IsEdge^{\oplus r}_{G}$. So by the guarantees of {\sc DT-Learn}, our algorithm correctly outputs ``Yes''. }

        In the \textbf{No case}, every vertex cover of $G$ has size at least $(1+\delta')k$. If $\eps_{\text{hyp}}>\eps$ then our algorithm for {\sc Vertex Cover} correctly outputs ``No''. Otherwise, assume that $\eps_{\text{hyp}}\le \eps$. Then, \Cref{lem:technical-xor} ensures that $(1+\delta)^rs<|T_{\text{hyp}}|$ and so our algorithm correctly outputs ``No'' in this case as well.
    % In the \textbf{yes} case, there is a vertex cover of size $\le k$ for $G$ and so 
    % \begin{align*}
    %     \dtsize(\ell\text{-}\IsEdge^{\oplus r}_{G_{\mathrm{yes}}})&= \dtsize(\ell\text{-}\IsEdge_{G_{\mathrm{yes}}})^r\tag{\Cref{thm:zero-error-xor}}\\
    %     &\le \left[(\ell+1)(k+m)+mn\right]^r\tag{\Cref{thm:ell-isedge-ub}}.
    % \end{align*}
    % Therefore, by the approximation guarantee of our learning algorithm, we have $|T|\le A\cdot\left[(\ell+1)(k+m)+mn\right]^r$ and the error is less than $\eps$. So our algorithm for vertex cover correctly outputs ``Yes''.

    % In the \textbf{no} case, every vertex cover of $G$ has size at least $(1+\delta')k$. If $\dist_{\mathcal{D}^{\otimes r}}(T,\ell\text{-}\IsEdge^{\oplus r}_{G})\ge \eps$, then our algorithm correctly outputs ``No''. Otherwise, assume that $\dist_{\mathcal{D}^{\otimes r}}(T,\ell\text{-}\IsEdge^{\oplus r}_{G})<\eps$. We'll show that $|T|>A\cdot\left[(\ell+1)(k+m)+mn\right]^r$ so that our algorithm correctly outputs ``No'' in this case as well. If we let $\delta\coloneqq A^{1/r}-1$, then the assumption of the theorem statement is that $\delta'>(\delta+8\eps^{1/r})d+\delta$. Thus, we can apply \Cref{lem:technical-xor} to get that
    % $$
    % A\cdot\dtsize(\ell\text{-}\IsEdge^{\oplus r}_{G_{\mathrm{yes}}})=(1+\delta)^r\dtsize(\ell\text{-}\IsEdge^{\oplus r}_{G_{\mathrm{yes}}})<\dtsize_{\mathcal{D}^{\otimes r}}(\ell\text{-}\IsEdge^{\oplus r}_{G_{\mathrm{no}}},\eps).
    % $$
    % Since $\left[(\ell+1)(k+m)+mn\right]^r=\dtsize(\ell\text{-}\IsEdge^{\oplus r}_{G_{\mathrm{yes}}})$ this ensures that our algorithm correctly outputs ``No'' in this case. 
\end{proof}

\begin{remark}[Why we require such sharp lower bounds in the proof of \Cref{thm:dt-learn-xor}]
\label[remark]{remark:sharp}
    A key step in the analysis of the correctness of our reduction is \Cref{lem:technical-xor}. Since our upper bound for $\ell$-$\IsEdge$ is of the form $s^r$, we require an equally strong lower bound of the form $(s')^r$. A weaker lower bound $(s')^{cr}$ for some $c<1$ would be insufficient, since the parameter $s$ would no longer separate the Yes and No cases in \Cref{lem:technical-xor}. 
\end{remark}



\subsection{Proof of \Cref{thm:main-general}}
By \Cref{thm:hardness of vertex cover}, there is a constant $\delta$ such that if {\sc Vertex Cover} can be approximated to within a factor of $1+\delta$ in time $t(n)$, then SAT can be solved in time $t(n\polylog n)$. Given an $n$-vertex graph with constant degree $d$, the reduction in \Cref{thm:dt-learn-xor} produces an instance of {\sc DT-Learn} in time $n^{O(r)}$. We choose $A=2^{\Theta(r)}$ in \Cref{thm:dt-learn-xor} so that $\frac{\delta}{2}>(A^{1/r}-1)d+A^{1/r}-1$ and $\eps=2^{-\Theta(r)}$ small enough so that $\frac{\delta}{2}>\eps^{1/r}\cdot 8d$. This ensures that our reduction from {\sc Vertex Cover} produces an instance of {\sc DT-Learn}$(s,2^{\Theta(r)}\cdot s,2^{-\Theta(r)})$ for $s=n^{O(r)}$. The algorithm guaranteed by the theorem statement solves {\sc DT-Learn}$(s,2^{\Theta(r)}\cdot s,2^{-\Theta(r)})$ in time $t(n^{O(r)}, 2^{O(r)})$. Therefore, by \Cref{thm:dt-learn-xor}, {\sc Vertex Cover} can be approximated to within a factor of $1+\delta$ in time $O(rn^2)\cdot t(n^{O(r)}, 2^{O(r)})$. The proof is completed by using the reduction from SAT to approximating {\sc Vertex Cover}.\hfill$\blacksquare$


\subsection{Proof of \Cref{thm:main}}
Let $C>1$ be the constant from the theorem statement. Let $r\ge 1$ be a large enough constant so that the $2^{O(r)}$ term in \Cref{thm:main-general} is greater than $C$. In this case, the error parameter $\eps=2^{-\Theta(r)}$ is also a small constant that depends on $C$. It follows that any polynomial-time algorithm solving the problem in the theorem statement can solve SAT in time $\Tilde{O}(rn^2)\cdot \poly(n^{O(r)},2^{O(r)})$ which is polynomial when $r$ is constant. Therefore, the task is NP-hard.\hfill$\blacksquare$


==> coresets.tex <==
\section{Coresets}

\begin{theorem}[Coresets for monotone functions]
\label{thm:coreset}
    For every monotone function $f:D\to\zo$ with $D\sse \zo^n$, there is a coreset $H\sse D$ of size $|H|=m\cdot\Sens(f)$ such that any decision tree computing $f$ over the coreset must have size at least $m$ where $m$ is the number of minterms of $f$.
\end{theorem}

\begin{proof}
    The coreset $H\sse D$ consists of all of the minterms and their sensitive neighbors:
    $$
    H\coloneqq \bigcup_{x\in\minterm(f)}\{x\}\cup\Sens(f,x).
    $$
    Let $T$ be a decision tree such that $T(x)=f(x)$ for all $x\in H$. We claim that $|T|\ge m$. If not, there are two minterms $x,x'$ which follow that same path $\pi$ in $T$. Since $x$ and $x'$ are distinct minterms, there is some coordinate on which they differ. Suppose $x$ is $1$ on the $i$th coordinate and $x'$ is $0$ on the $i$th coordinate. By definition, since $x$ is a minterm it must be sensitive on the $i$th coordinate. But the path $\pi$ doesn't query the $i$th coordinate, so $x^{\oplus i}\in H$ follows the same path $\pi$ but is a $0$-input, thereby yielding an error.
\end{proof}

\begin{theorem}[Alternative formulation]
    For every monotone function $f:D\to\zo$ with $D\sse \zo^n$, there is a coreset of size $s$ such that 
    \begin{enumerate}
        \item there is a decision tree of size $s$ computing $f$ over the coreset; and
        \item every decision tree computing $f$ over the coreset must have size at least $\frac{s}{n}$.
    \end{enumerate}
\end{theorem}


\begin{theorem}[Distributional lower bound for coresets]
    Let $f,H,$ and $m$ be as in \Cref{thm:coreset}. Then, there is a distribution $\mathcal{D}$ such that
    $$
    |T|\ge (1-\Sens(f)\eps)m
    $$
    for all decision trees $T$ satisfying $\error_{\mathcal{D}}(f,T)\le \eps$.
\end{theorem}



==> intro.tex <==
%!TEX root = paper.tex


% \title{Superconstant inapproximability of decision tree learning \vspace{10pt}}



%\author{ 
%Caleb Koch \vspace{6pt} \\ 
%{\small {\sl Stanford}} \and 
%\hspace{5pt} Carmen Strassle \vspace{6pt} \\
%\hspace{5pt} {\small {\sl Stanford}} \and 
%Li-Yang Tan \vspace{6pt}  \\
%\hspace{-10pt} {\small {\sl Stanford}}
%}

% \date{\today}

% \include{intro-new}


% \begin{abstract}
% \end{abstract} 

% \thispagestyle{empty}
% \newpage 


% \tableofcontents
% \thispagestyle{empty}
% \newpage 

% \setcounter{page}{1}

% \paragraph{High level pitch:} We prove it is NP-hard to approximate the problem of decision tree minimization given a dataset to within any constant factor. Under the assumption $\mathrm{NP}\not\sse \mathrm{DTIME}(n^{\polylog n})$, we obtain hardness of approximating within a factor of $n^{o(1)}$. Our results improve on the previous best known hardness of approximation factor of $(1+\delta)$ for some small constant $\delta>0$. As an application of our result, we give new lower bounds for learning decision trees with queries. Our application relies on a new XOR lemma for decision tree size which may be of independent interest. Along the way, we also recover via a simpler proof the recent constant-error hardness of learning decision trees with queries from Koch, Strassle, and Tan (2023).


% \section{Notes and TODOs}
% \begin{enumerate}
%     \item Finishing working out the learning consequences of the XOR lemma
%     \item Work out consequences for DT minimization over a dataset. Remark how this is a strict strengthening of Sieling's hardness of approximating \textit{exact} DT minimization to within a factor of $2^{(\log n)^\delta}$
%     \item Show that our techniques recover the constant-error hardness of learning DTs from KST23 via a different and simpler proof. Also, as a technical aside, I think our techniques get hardness directly from vertex cover instead of having to go through $\alpha$-partial vertex cover.
%     \item Generalize Shaltiel's counterexample to decision tree size to show that one cannot hope to extend our XOR lemma to work for all functions (this justifies our assumptions/specialization to IsEdge).
%     \item Remark that Drucker gives a DPT for decision tree size. One can show that DPTs for DT size imply XOR lemmas for DT size and so Drucker's result also yields an XOR lemma for DT size. However, we can show that Drucker's XOR lemma applied to IsEdge is insufficient for our purposes (essentially: his LB gives something like $(k+m)^{0.001 r}$ while we need a much stronger $(k+0.999m)^r$ lower bound). IRW94 also gives a DPT for DT size but this is also too weak for our setting (theirs does not blow-up the size). 
%     % \item Give an explicit construction of an upper bound for $\IsEdge^{\oplus r}$ which shows that our XOR lemma is nearly tight (in particular, the $2^{-\Theta(r)}$ lossk++__ in error is necessary). 
% \end{enumerate}

% \textbf{Other questions as of January}

% \begin{enumerate}
%     \item (An XOR lemma for coresets) Suppose there is a coreset for monotone $f$ for size $s$ to constant error, is there a coreset of size $s^r$ for $f^{\oplus r}$ for size $s^r$ and error $\eps=\Theta(2^{-r})$
%     \item Can we generically lift DT-minimization hardness wrt to monotone functions into hardness of learning decision trees with query (possibly to inverse-poly error)?
% \end{enumerate}


\cleardoublepage


\section{Overview}

\paragraph{Learning decision trees with queries}{
We are interested in the following learning task:

\begin{tcolorbox}[colback = white,arc=1mm, boxrule=0.25mm]
\vspace{3pt} 
{\sc DT-Learn$(s,s',\eps)$:}  Given queries to an unknown function $f : \zo^n \to \zo$, random samples from a distribution $\mathcal{D}$ over $\zo^n$, parameters $s,s'\in \N$ and $\eps \in (0,1)$, and the promise that $f$ is a size-$s$ decision tree under $\mathcal{D}$, construct a size-$s'$ decision tree $T$ that is $\eps$-close to $f$ under $\mathcal{D}$.
\vspace{3pt}
\end{tcolorbox}
\medskip
}
When $s=s'$, DT-Learn$(s,s',\eps)$ is also known as \textit{strongly}-proper learning. Previously, we showed hardness when $s$ is very close to $s'$. We refer to the task DT-Learn$(s,s',\eps)$ for $s'\gg s$ as \textit{weakly}-proper learning. The bigger $s'$ is, the weaker the learner. Naturally, if we assume a learner is weak rather than strong, it can only be harder to prove lower bounds against.

\begin{theorem}[KST 2023]
    \label{thm:focs-main}
    There are constants $\eps>0$ and $\delta>0$ such that {\sc DT-Learn}$(s,(1+\delta)s, \eps)$ is $\mathrm{NP}$-hard.
\end{theorem}

This hardness result is rather limited, it says nothing about, e.g. the complexity of DT-Learn$(s,2s,\eps)$. The goal of this work is to better understand the regimes for which {\sc DT-Learn}$(s,s',\eps)$ remains hard. We can show that the problem remains hard to solve even when $s'$ is much larger than $s$.

\begin{theorem}[Constant-error hardness of {\sc DT-Learn}]
    \label{thm:constant-error-hardness}
    For all constants $c>1$, there is a constant $\eps>0$ such that {\sc DT-Learn}$(s,cs,\eps)$ where the unknown target is a polynomial-size decision tree is $\mathrm{NP}$-hard.
\end{theorem}

In fact, our theorem gives a generic tradeoff between how large $s'$ can be relative to the error while still remaining hard. 

\begin{theorem}[A general reduction from {\sc VertexCover} to {\sc DT-Learn}]
    \label{thm:size-error-tradeoff}
    For all $r\ge 1$ and constant $\delta>0$, there is a reduction running in time $n^{O(r)}$ from $(1+\delta)$-approximating \textsc{VertexCover} on $n$-vertex graphs to {\sc DT-Learn}$(s,2^{\Theta(r)}\cdot s,2^{-\Theta(r)})$ where the unknown target function is over $N=rn^2$ variables and is a size $s=n^{O(r)}$ decision tree.
\end{theorem}

As soon as $r$ is superconstant, this hardness result requires learning decision trees to subconstant error. However, it can yield hardness even against even more weakly proper learners. For example, choosing $r=(\log s)^{\gamma}$ for an appropriate choice of $\gamma<1$ yields hardness of {\sc DT-Learn}$(s,s^{1+o(1)},2^{-(\log s)^{\gamma}})$ assuming $\mathrm{NP}\not \sse \text{DTIME}(n^{\polylog (n)})$.


\section{Our approach}
\paragraph{Notation}{
For a function $f:\zo^n\to\zo$, distribution $\mathcal{D}$ over $\zo^n$, and $\eps\in (0,1)$, write
$$
\dtsize_{\mathcal{D}}(f,\eps)
$$
to denote the size of the smallest DT that computes $f$ with error $\eps$ over $\mathcal{D}$. 
}

\paragraph{Lower bounding the decision tree complexity of $\ell\text{-}\IsEdge$.}{
Previously, we obtained \Cref{thm:focs-main} via the $\ell\text{-}\IsEdge$ function. We defined a hard distribution $\ell\text{-}\mathcal{D}$ over inputs and showed that even approximating it to constant error requires large decision tree size:

\begin{theorem}[DT complexity of $\ell\text{-}\IsEdge$]
    \label{thm:l-isedge-lb}
    Let $G$ be an $m$-edge graph and $\alpha\in (0,1)$, then
    $$
    \dtsize_{\ell\text{-}\mathcal{D}}(\ell\text{-}\IsEdge, \alpha)\ge (\ell+1)\cdot (k+(1-16\alpha)m)
    $$
    where $k$ is the $\alpha$-partial vertex cover size of $G$.
\end{theorem}
}

\paragraph{Lower bounding the decision tree complexity of $\ell\text{-}\IsEdge^{\oplus r}$.}{
In order to prove \Cref{thm:constant-error-hardness,thm:size-error-tradeoff}, we consider the function $\ell\text{-}\IsEdge^{\oplus r}$, the XOR of $r$ copies of $\ell\text{-}\IsEdge$. We define a hard distribution $\mathcal{D}$ and show that this function remains hard to approximate:

\begin{theorem}[Hardness for computing $\ell\text{-}\IsEdge^{\oplus r}$ (informal, see \Cref{thm:ellisedge-lb-xor} for the exact statement)]
    \label{thm:l-isedge-xor-lb-informal}
    Let $T$ be a decision tree for $\ell\text{-}\IsEdge^{\oplus r}$, then
    $$
    \dtsize_{\mathcal{D}}(\ell\text{-}\IsEdge^{\oplus r},\alpha)\ge \Bigg[(\ell+1)(k+(1-\alpha^{1/r})m)\Bigg]^r.
    $$
\end{theorem}
}
\paragraph{How \Cref{thm:l-isedge-xor-lb-informal} yields better learning hardness.} {
The basic idea for \Cref{thm:focs-main} is that a small constant gap in vertex cover complexity translates into a small constant gap in the decision tree complexity of $\ell\text{-}\IsEdge$. \Cref{thm:l-isedge-lb} shows that this gap is preserved even with respect to the decision tree complexity of \textit{approximating} $\ell\text{-}\IsEdge$. This way, if a decision tree learner can find a close-to-optimal decision tree that approximates $\ell\text{-}\IsEdge$, it can be used to solve vertex cover merely by inspecting the size of the decision tree it learns. By taking the XOR of many copies of $\ell\text{-}\IsEdge$, we expect its decision tree size to blow-up. The hope is that this blow-up will amplify the constant gap in decision tree size. Roughly speaking, \Cref{thm:l-isedge-lb} shows a gap of $s$ versus $(1+\delta)s$ in the size of $\ell\text{-}\IsEdge$ which gets amplified to a gap of $s^r$ versus $(1+\delta)^r s^r$ in the size of approximating $\ell\text{-}\IsEdge^{\oplus r}$ to error $\alpha=2^{-\Theta(r)}$ (this is inexact as technically the difference of $s$ versus $(1+\delta)s$ depends on the error of the decision tree computing $\ell\text{-}\IsEdge$; we are hiding the error dependence for simplicity). 
}

The rest of this write-up is dedicated to proving \Cref{thm:l-isedge-xor-lb-informal}. We develop a generic framework for proving lower bounds against the size of decision trees approximating a function over a ``canonical hard distribution''. We then consider how the framework behaves relative to XORing many copies of a function together. Finally, we apply the framework to $\ell\text{-}\IsEdge^{\oplus r}$ in order to obtain \Cref{thm:l-isedge-xor-lb-informal}.

\paragraph{\Cref{thm:l-isedge-xor-lb-informal} is not generalizable.} \Cref{thm:l-isedge-xor-lb-informal}, taken together with an upper bound for the decision tree complexity of $\ell\text{-}\IsEdge$\carnote{figure out which upper bound exactly}, yields a strong XOR lemma for the function $\ell\text{-}\IsEdge$. In particular, 
\begin{align*}
    \dtsize_{\mathcal{D}}(\ell\text{-}\IsEdge^{\oplus r},2^{-\Theta(r)})\ge \Bigg[\dtsize_{\ell\text{-}\mathcal{D}}(\ell\text{-}\IsEdge, \eps)\Bigg]^r
\end{align*}
where $\eps>0$ is some small constant. A statement of this form does \textit{not} hold for general $f$. To prove that strong XOR lemmas cannot hold in general, \cite{Sha04} constructs a specific function, which we call $\mathsf{Shal}$, with the following behavior:
\begin{align*}
    \dtsize_{\mu^{\oplus r}}(\mathsf{Shal}^{\oplus r},2^{-\eps r})\le \Bigg[\dtsize_{\mu}(\mathsf{Shal}, \eps)\Bigg]^{\eps r}.
\end{align*}

\newpage



